Can I Trust My Simulation Model? Measuring the Quality of Business Process Simulation Models

Business Process Simulation (BPS) is an approach to analyze the performance of business processes under different scenarios. For example, BPS allows us to estimate what would be the cycle time of a process if one or more resources became unavailable. The starting point of BPS is a process model annotated with simulation parameters (a BPS model). BPS models may be manually designed, based on information collected from stakeholders and empirical observations, or automatically discovered from execution data. Regardless of its origin, a key question when using a BPS model is how to assess its quality. In this paper, we propose a collection of measures to evaluate the quality of a BPS model w.r.t. its ability to replicate the observed behavior of the process. We advocate an approach whereby different measures tackle different process perspectives. We evaluate the ability of the proposed measures to discern the impact of modifications to a BPS model, and their ability to uncover the relative strengths and weaknesses of two approaches for automated discovery of BPS models. The evaluation shows that the measures not only capture how close a BPS model is to the observed behavior, but they also help us to identify sources of discrepancies.

==> sm.tex <==



ServiceMiner (SM) operates in three steps, namely data preprocessing, 
data enhancement, and model learning.
First, event data goes through preprocessing such as data cleaning, and 
dummy encoding of categorical features. For data enhancement, new data attributes that capture trend, and seasonality, as well as system congestion are created using methods described in~\cite{senderovich2019congestion}.
In the model learning step, SM uses three techniques: process discovery (the main
task of process mining), queue mining (learning of queueing building blocks from data), and 
machine learning (to boost the accuracy of arrival and activity time genration). For process discovery, SM mines a Markov chain, estimating the routing probabilities 
between pairs of nodes. An abstraction mechanism allows for filtering out of rare activities, paths, and transitions,
based on the created graph. Next, using queue mining, the various queueing building blocks are fitted from data. The basic version of queue mining is described in~\cite{senderovich2016conformance}; ServiceMiner uses advanced versions of these techniques.
The model that results from queue mining is a queueing network with Markovian routing. 
Lastly, we apply machine learning methodology that uses congestion related features that come from queueing theory,
which, via cross-validation, leads to accuracy improvements when generating arrival and activity duration.

